Safe Policies for Reinforcement Learning via Primal-Dual Methods

In this paper, we study the learning of safe policies in the setting of reinforcement learning problems. This is, we aim to control a Markov Decision Process (MDP) of which we do not know the transition probabilities, but we have access to sample trajectories through experience. We define safety as the agent remaining in a desired safe set with high probability during the operation time. We therefore consider a constrained MDP where the constraints are probabilistic. Since there is no straightforward way to optimize the policy with respect to the probabilistic constraint in a reinforcement learning framework, we propose an ergodic relaxation of the problem. The advantages of the proposed relaxation are threefold. (i) The safety guarantees are maintained in the case of episodic tasks and they are kept up to a given time horizon for continuing tasks. (ii) The constrained optimization problem despite its non-convexity has arbitrarily small duality gap if the parametrization of the policy is rich enough. (iii) The gradients of the Lagrangian associated with the safe-learning problem can be easily computed using standard policy gradient results and stochastic approximation tools. Leveraging these advantages, we establish that primal-dual algorithms are able to find policies that are safe and optimal. We test the proposed approach in a navigation task in a continuous domain. The numerical results show that our algorithm is capable of dynamically adapting the policy to the environment and the required safety levels.

==> gradient.tex <==
%!TEX root = root.tex

\section{Gradient Ascent for Safe Learning}\label{sec_gradient}
%


==> introduction.tex <==
%!TEX root = root.ted


%The goal of the agent is thus to find a control law that maximizes the value function of the MPD, i.e., the expectation of the cumulative rewards \cite{sutton1998reinforcement}.


\section{Introduction}\label{sec_intro}
%
Markov Decision Processes~(MDP's)~\cite{howard1964dynamic} are stochastic control processes used ubiquitously to study robotic systems~\cite{kober2013reinforcement}, control problems~\cite{shreve1978alternative}, and financial models~\cite{rasonyi2005utility}. When the models are available, optimal control laws---or \emph{policies}---can be obtained for these processes using dynamic programming~\cite{bertsekas1996neuro}. In contrast, when the underlying MDP is unknown or the system is too complex, the policy needs to be learned from samples of the system. Typically, this is done by assigning an instantaneous \emph{reward} to the system actions that describes the task to be learned. These rewards can be aggregated over a trajectory to determine cumulative rewards. Since the instantaneous rewards depend both on the state and on the actions selected based on the current state, cumulative rewards are a measure of the quality of the decision making policy of the agent. The objective of the agent is therefore to find a policy that maximizes the expectation of the cumulative rewards, which is known as the \emph{value function}~(or the \emph{Q-function}) of the MDP~\cite{sutton2018reinforcement}.

Solutions to these problems can be roughly divided among those that learn the Q-function to then chose for any given state the action that maximizes the function \cite{watkins1992q}, and those that attempt to directly learn the optimal policy \cite{williams1992simple,sutton2000policy}. \blue{A drawback of Q-learning \cite{watkins1992q} for continuous state-action spaces\textemdash and any other algorithm that learns Q-functions for that matter\textemdash is that even after trainging, the selection of each action amounts to solving a nonconvex optimization problem. } 
This motivates development of algorithms that attempt to learn the optimal policy directly by performing (stochastic) gradient ascent on the value function with respect to a policy variable \cite{williams1992simple, sutton2000policy}.


A notable drawback of these methods is that it is not always suitable for learning dangerous, risky tasks~\cite{heger1994consideration, mihatsch2002risk, geibel2005risk}. Indeed, many applications require robust control strategies which also take into account, for instance, the variance of the accumulated reward to avoid situations in which its value on a specific realization of the process is considerably worse than its mean. Consider the case of a self-driving car deployed in an urban environment. To reach a destination as fast as possible, the optimal policy may be such that it makes risky maneuvers, such as driving close to other cars or crossing pedestrians. Due to the random components in the vehicle actions and the behavior of other cars and pedestrians, collision avoidance cannot be guaranteed.

Strategies used to overcome this limitation can be mapped to four approaches. The first formulates a robust problem in which the policy is optimized over its worst case return~\cite{heger1994consideration, coraluppi1999risk}. However, these techniques generally yield policies too conservative for the average scenario and make it hard to control the trade-off between safety and performance. The second family of solutions propose to modify the instantaneous reward function so as to reflect a subjective measure balancing risk and task learning~\cite{howard1972risk, geibel2005risk}. Although this approach makes the risk-performance trade-off more transparent, it requires this balance to be hand-tuned, an often time consuming and challenging task that requires application\textemdash and domain-specific expert knowledge, as shown in \cite{tessler2018reward,leike2017ai,mania2018simple}. Moreover, implicit interference between the goals may lead to training plateaus as they compete for resources in the policy~\cite{schaul2019ray}. What is more, the function of the reward is to inform the goal of the agent, not prior knowledge on how to complete it. Indeed, ``the reward signal is your way of communicating to the robot \emph{what} you want it to achieve, not \emph{how} you want it achieved''~\cite[Section~3.2]{sutton2018reinforcement}. The third approach addresses this issue by modifying the learning procedure instead of the the reward. By performing safe exploration~\cite{moldovan2012safe,turchetta2016safe,koller2018learning}, the agent learns from safe trajectories and is therefore biased to learn safe policies.

The last class of solutions addresses the issue of safety by including explicit constraints in the optimization problem used to learn the policy~\cite{geibel2006reinforcement, kadota2006discounted, delage2010percentile, di2012policy, hutter2002self, chow2017risk}. This is the approach taken in this paper. These constraints are typically probabilistic in nature, in the sense that they require certain requirements to hold with some given minimum probability. These requirements can involve, for instance, lower bounds on the value function or additional value functions~\cite{kadota2006discounted, geibel2006reinforcement, delage2010percentile}, thus relaxing the worst case approach from~\cite{heger1994consideration, coraluppi1999risk}, or arbitrary functions of the state-action space~\cite{chow2017risk, achiam2017constrained}. These constrained learning problems are solved by using regularization and relaxations so they can be written as linear programs~\cite{hutter2002self, geibel2006reinforcement}, by leveraging approximate trust region methods~\cite{achiam2017constrained}, or by applying primal-dual algorithms~\cite{chow2017risk}. A comprehensive review of this topic can be found in~\cite{garcia2015comprehensive}.
%\cite{di2012policy} Mean variance trade-off

In this work, we formulate safety constraints by imposing a lower bound on the probability of remaining in the safe set for all times. We then propose relaxations for the finite and infinite time operations~(Section~\ref{sec_safe_learning}) and provide guarantees on the ergodic safety of policies learned using our relaxed formulations~(Section~\ref{sec_safety_guarantees}). Namely, we show that these relaxations do not affect the safety level of the finite horizon problem and establish a safe operation horizon in the infinite case. The relaxation proposed has two main advantages. On the one hand, we establish in Section~\ref{sec_zdg} that the safe-learning problem, despite its non convexity has zero duality gap. The latter implies that the trade-offs expressed by different weights in the risk aware rewards are the same as those expressed by the probability specifications, in the sense that they trace the same Pareto front. Nevertheless, the relationship between weights and specifications is not trivial and specifying the constrained problem is often considerably simpler. The second advantage of the proposed relaxation is that it provides an easy expression to compute stochastic approximations of the gradient of the Lagrangian associated to the safe learning problem~(Section~\ref{sec_pd}). The latter allows us to run dual or primal-dual algorithms to solve the safe learning problem, where we leverage the zero duality gap results to show convergence. Other than concluding remarks, the paper finishes with numerical experiments in which we show that primal-dual methods are able to automatically adjust the trade-off between goal and safety~(Section~\ref{num_results}).


==> pd.tex <==
%!TEX root = root.tex

\section{Primal-Dual Algorithm}\label{sec_pd}
% 
As previously stated the advantage of working in the dual domain is that the dual function~\eqref{eqn_parametric_dual_function} is convex and therefore gradient descent (or its stochastic variants) allows us to solve the safe learning problem~\eqref{P:parametric}. \red{BTW, primal dual has been used in the literature extensivelly in optimization in general and specifically also in RL. Here we just provide a convergence guarantee to the solution of the primal} 

For completeness we start by considering plain dual gradient descent. Let $\nabla_\lambda d_\theta(\lambda)$ be the gradient of the dual function, then dual gradient descent is defined by the following update rule
%
\begin{equation}\label{eqn_pure_gradient_descent}
\lambda^{k+1} = \left[\lambda^k-\eta_\lambda \nabla_\lambda d_\theta(\lambda^k)\right]^+,
  \end{equation}
%
where $\eta_\lambda>0$ is a step-size and the operation $\left[\cdot\right]^+$ denotes a projection onto the positive orthant of $\mathbb{R}^m$. The latter algorithm is ensured to converge to a neighborhood of the dual optimum \cite[pp 43-45]{bertsekas1999nonlinear}. In addition, the gradient of the dual function can be computed using Dankin's Theorem (see e.g. \cite[Chapter 3]{bertsekas15c}) by evaluating the constraints in the original problem \eqref{P:parametric} at the primal maximizer of the Lagrangian, i.e.,
%
\begin{equation}\label{eqn_dual_gradient}
\nabla_\lambda d_\theta(\lambda^k) = U(\theta^\star(\lambda^k)) -c_i,
\end{equation}
%
where $\theta^\star(\lambda^k) := \argmax_{\theta\in\mathbb{R}^d}\ccalL(\lambda^k,\theta)$. As discussed in Section \ref{sec_safe_learning} computing the maximizer of the Lagrangian for a given $\lambda$ is equivalent to maximizing the expected discounted control cost for the risk aware reward~\eqref{eqn_risk_aware_reward} and~\eqref{reward_constrained}.

Depending on the framework of interest this maximization can be done using several techniques. In the case of model-free scenarios, classic reinforcement learning algorithms such as policy gradient~\cite{williams1992simple,sutton2000policy,paternain2018stochastic} or actor-critic methods~\cite{konda2000actor} can be used. Since these algorithms are gradient based they are not guaranteed to converge to a global maximum. However, because they achieve good performance, it is not unreasonable to assume that they converge to a solution with small suboptimality. A possibility to formalize this idea, is to assume that the local maxima of the Lagrangian are not too different in value than the global maxima. 
%
  \begin{assumption}\label{assumption_neural_network}
Let $\ccalL_\theta(\theta,\lambda)$ with $\lambda\in\mathbb{R}^m_+$ be the Lagrangian associated to \eqref{P:parametric}. Denote by $\theta^\star(\lambda),\theta^\dagger(\lambda)\in\mathbb{R}^d$ the maximum of $\ccalL_\theta(\theta,\lambda)$ and a local maximum respectively achieved by a generic reinforcement learning algorithm. Then, there exists $\beta>0$ such that for all $\lambda\in\mathbb{R}^m_+$ it holds that $\ccalL_\theta(\theta^\star(\lambda),\lambda) \leq \ccalL_\theta(\theta^\dagger(\lambda),\lambda)+\beta$.
\end{assumption}
  %
  Notice that the previous assumption means that we are able to solve the regularized unconstrained problem approximately. This means that the parameter at time $k+1$ satisfies 
%
\begin{equation}\label{eqn_primal_max}
\ccalL_\theta(\theta^{k+1},\lambda^k) \approx \max_{\theta\in\mathbb{R}^d} \ccalL_\theta(\theta,\lambda^k).
\end{equation}
%
{Then, the dual variable is updated following the gradient descent scheme suggested in~\eqref{eqn_pure_gradient_descent}, where we replace the gradient of the dual function given in \eqref{eqn_dual_gradient} by the approximation based on the primal variable available $\theta^{k+1}$. This yields the following update 
%
\begin{equation}\label{eqn_gradient_descent}
\lambda^{k+1} =\left[\lambda^k - \eta_\lambda \left(U(\theta^{k+1})-c\right)\right]_+.
  \end{equation}
%
The algorithm given by~\eqref{eqn_primal_max}--\eqref{eqn_gradient_descent} is summarized for convenience under Algorithm~\ref{alg_dual_descent}.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% A L G O R I T H M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
  \caption{Dual Descent}
  \label{alg_dual_descent} 
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require $\eta_\lambda$
 \State \textit{Initialize}: $\theta^0 = 0$, $\lambda^0 = 0$
  \For {$k=0,1\ldots$}
  \State Compute a primal approximation via an RL algorithm to get $\theta^{k+1}$ such that 
   \begin{align*}
      \ccalL_{\theta}(\theta^{k+1},\lambda^k) \approx \max \ccalL_{\theta}(\theta,\lambda^k)
  \end{align*}

  \State Compute the dual ascent step 
  \begin{align*}
  \lambda^{k+1} = \left[\lambda^k-\eta_\lambda \left(U(\theta^{k+1})-c\right)\right]_+
  \end{align*}
  \EndFor
 \end{algorithmic}
 \end{algorithm}
%%
%
The previous algorithm relies on the fact that the approximation of the subgradient used in the above equation does not differ much from the gradient \eqref{eqn_dual_gradient}.  We claim in the following proposition that this is the case. In particular, we establish that the constraint evaluation does not differ from the subgradient in more than $\beta$, the error on the primal maximization defined in Assumption \ref{assumption_neural_network}. 
%
\begin{proposition}\label{prop_subgradient}
  Under Assumption \ref{assumption_neural_network}, the constraint in \eqref{P:parametric} evaluated at a local maximizer of the Lagrangian $\theta^\dagger(\lambda)$ approximate the subgradient of the dual function \eqref{eqn_parametric_dual_function}. In particular it follows that
  %
  \begin{equation}
    d_\theta(\lambda) - d_\theta(\lambda_\theta^\star) \leq  \left(\lambda-\lambda_\theta^\star\right)^\top\left( U(\theta^\dagger(\lambda))-c\right)+\beta.
  \end{equation}
  %
  \end{proposition}
%
\begin{proof}
See Appendix \ref{proof_subgradient}.
  \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONVERGENCE THEOREM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The previous proposition is key in establishing convergence of primal-dual algorithms since it allows us to claim that the dual updated is an approximation of a dual descent step. We formalize this result next and we establish a maximum number of dual steps required to achieve a desired accuracy.
%

\begin{theorem}\label{T:convergence}
  %
Let $\theta$ be an $\epsilon$-universal parametrization of $\ccalP(\ccalS)$ according to Definition \ref{def_universal_param}, $B_r$ be a bound on the reward~$r(s,a)$  and~$\gamma\in(0,1)$ be the discount factor. Then, if Slater's conditions hold for~\eqref{P:parametric}, under Assumption \ref{assumption_neural_network} and for any $\varepsilon>0$, the sequence of updates of Algorithm \ref{alg_dual_descent} with step size $\eta_\lambda$ converges in $K>0$ steps, with 
  %
 \begin{equation}
          K \leq \frac{\left\|\lambda^0-\lambda_\theta^\star\right\|^2}{2\eta_\lambda \varepsilon},
 \end{equation} 
%
 to a neighborhood of $P^\star$ \textemdash the solution of \eqref{P:constrainedRL} \textemdash satisfying
  %
  \begin{equation}\label{eqn_convergence_neighborhood}
P^\star-\left(B_{r}+\left\|\lambda^\star\right\|_1\right)\frac{\epsilon}{1-\gamma}\leq     d_{\theta}(\lambda^K)\leq  P^\star+\eta_\lambda\frac{B}{2}+\beta+\varepsilon.
  \end{equation}
  %
{where~$B =\sum_{i=1}^m\left( B_r/(1-\gamma)-c_i\right)^2$} and~$\lambda^\star$ is the solution of \eqref{P:dualRL}.
  %
\end{theorem}
%
\begin{proof}
  See Appendix \ref{proof_convergence}.
  \end{proof}
The previous result establishes a bound on the number of dual iterations required to converge to a neighborhood of the optimal solution. Notice that its size depends on the representation ability of the parametrization chosen, and the goodness of the solution of the maximization of the Lagrangian. \blue{The bound on the number of iterations required is linear with the inverse of the desired accuracy $\varepsilon$ and it quantifies exactly the overhead solving the dual problem as compared to solving the risk aware optimal control problem for a hyperparameter $\lambda$ that needs to be hand-tuned as we have discussed in Section \ref{sec_safe_learning}. To complete this discussion we have in fact introduced two new parameters, the initial condition $\lambda_0$ and the step-size $\eta_\lambda$. Notice that the first parameter does not need to be tuned since the convergence is guaranteed for any initial condition. \red{What about the step-size?}}  

\red{Notice that without our result convergence to dual solution has been established before I guess, what we bring in the mix is the fact that we are actually converging to the optimizer.}  
%

Since the cost of running policy gradient or actor-critic algorithms until convergence before updating the dual variable might result in an algorithm that is computationally prohibitive, an alternative that is common in the context of optimization is to update the primal and dual variables in parallel \cite{arrow_hurwicz}. This idea can be applied in the context of reinforcement learning as well, where a policy gradient \textemdash or actor-critic as in  \cite{bhatnagar2012online, tessler2018reward}\textemdash update is followed by an update of the multipliers along the direction of the constraint violation. In these algorithms the update on the policy is on a faster scale than the update of the multipliers, and therefore they operate, from a theoretical point of view, as dual descent algorithms (cf., Algorithm \ref{alg_dual_descent}). In particular, the proofs in \cite{bhatnagar2012online, tessler2018reward} rely on the fact that this different time-scale is such that allows to consider the multiplier as constant. In particular this implies that the maximization in \eqref{eqn_primal_max} is replaced by a gradient ascent step
%
\begin{equation}\label{eqn_first_grad_ascent}
  \theta^{k+1} = \theta^k + \eta_{\theta} \nabla_\theta \ccalL(\theta^k,\lambda^k), 
  \end{equation}
%
where $\eta_\theta>0$ is the step-size of the primal ascent and it is required to be on a faster time-scale that the dual step, i.e., $\eta_{\theta}\gg \eta_\lambda$. 


Notice that the computation of the expressions \eqref{eqn_first_grad_ascent} and \eqref{eqn_gradient_descent} is not straightforward since they require the computation of expectations. In the case of $\nabla_\lambda \ccalL(\theta,\lambda)$ we are required to compute the expectation of the sum of the constraints as shown in \eqref{eqn_constraint_indicator} and \eqref{eqn_pure_gradient_descent}. The computation of the gradient with respect to the primal variable $\theta$ is more convoluted and it requires that we resort to the Policy Gradient Theorem \cite{sutton2000policy}. Let us define
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% A L G O R I T H M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
  \caption{Stochastic Primal-Dual for Safe Policies}
  \label{alg_pd} 
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require $\theta^0,\lambda^0,T, \eta_\theta,\eta_\lambda, \delta, \epsilon$
 %\State \textit{Initialize}: $\hat{Q} = 0$, $s_0 = s$, $a_0 =a$
 % \State Draw an integer $T_Q$ form a geometric distribution with parameter $\gamma$, $P(T_Q = t) = (1-\gamma)\gamma^t$
% \\ \textit{LOOP Process}
  \For {$k = 0,1,\ldots $}
  \State Simulate a trajectory with the policy $\pi_{\theta^k}(\bbs)$
  \State Estimate primal gradient $\hat{\nabla}_\theta\ccalL(\theta^k,\lambda^k)$ as in \eqref{eqn_stochastic_primal}
  \State Estimate dual gradient $\hat{U}(\theta^k)-s$ as in \eqref{eqn_stochastic_dual}
  \State Update primal variable
  $$
  \theta^{k+1} = \theta^k+ \eta_{\theta} \hat{\nabla}_\theta\ccalL(\theta^k,\lambda^k)
    $$
    \State Update dual variable
  $$
  \lambda^{k+1} = \left[\lambda^k+ \eta_{\lambda}\left(\hat{U}(\theta^k)-c\right)\right]_+
    $$
  \EndFor
% \Return $\theta$, $s_{T_Q}$ 
 \end{algorithmic}
 \end{algorithm}
%      
%
\begin{equation} \label{eqn_cum_reward_finite}
R_{T}^{\lambda}(\bbs,\bba) = \sum_{t=0}^T r_\lambda(s_t,a_t),
\end{equation} 
%
\begin{equation} \label{eqn_cum_reward_infinite}
R^{\lambda}_{\infty}(\bbs,\bba) = \sum_{t=0}^\infty \gamma^tr_\lambda(s_t,a_t)
\end{equation}
%
where $r_\lambda(s_t,a_t)$ is the reward defined in defined in \eqref{reward_constrained} for a given Lagrange multiplier $\lambda\in \mathbb{R}_+$. Further, define $\rho_{\theta,T}(s) = \sum_{t=0}^T p(s_t=s|s_0)/T$ and $\rho_{\theta,\infty}(s) = \sum_{t=0}^\infty \gamma^t p(s_t=s|s_0)$ and the corresponding $Q$-functions
  %
  \begin{equation}
    Q_{T/\infty}^\lambda(s,a) = \mathbb{E}\left[R^\lambda_{T/\infty}(\bbs,\bba)| s_0=s, a_0 =a\right].
    \end{equation}
%
  Then the gradient of the Lagrangian \eqref{eqn_lagrangian} with respect to the parameters of the policy $\theta$ for both formulations yields \cite{sutton2018reinforcement}
%
    \begin{equation}\label{eqn_primal_gradient}
 \nabla_\theta \ccalL(\theta,\lambda) =  \mathbb{E}_{a\sim\pi_{\theta}(a|s),s\sim \rho_\theta(s)}\left[Q^\lambda(s,a) \nabla_{\theta}\log \pi_{\theta}(a|s) \right].
      \end{equation}
    %
In both the expression for the gradient with respect to the primal and the dual variables we require to compute expectations with respect to the trajectories of the system. To avoid sampling a large number of trajectories, one can instead use stochastic approximations \cite{robbins1951stochastic}. This is, with one sample trajectory, one can compute in the case of the finite horizon problem estimates of $U(\theta^k)$ as
    %
    \begin{equation}\label{eqn_stochastic_dual}
      \hat{U}(\theta^k) =\sum_{t=0}^Tr_{\lambda}(s_t,a_t),
      \end{equation}
    %
    and
    \begin{equation}\label{eqn_stochastic_primal}
\hat{\nabla}_{\theta}\ccalL(\theta^k,\lambda^k) = R^{\lambda^k}(\bbs,\bba)\nabla_{\theta}\log \pi_{\theta^k}(a_0|s_0).
      \end{equation}
    %
    In cases where the horizon is finite, the previous expressions can be computed without any additional steps and they yield unbiased estimates of the quantities that they estimate. However, for the infinite horizon case, one would require an infinite trajectory for the later to hold. An alternative, and given the equivalence between the finite and infinite time horizon problem discussed in Remark 1 is to sample a horizon from a geometric distribution. By computing the expressions in \eqref{eqn_stochastic_primal} and \eqref{eqn_stochastic_dual} over the randomly drawn horizon the estimates obtained are unbiased \cite{paternain2018stochastic}. The stochastic primal-dual algorithm is summarized in Algorithm \ref{alg_pd} and in the next section we show how it can be used to safely navigate an obstacle-ridden space. A different alternative to computing \eqref{eqn_stochastic_primal} is to use actor-critic updates as done in \cite{bhatnagar2012online, tessler2018reward}. Actor-critic methods estimate the gradient with less variance and therefore they enjoy better convergence guarantees. In this work we limit the development to the version of the algorithm given in \eqref{eqn_stochastic_primal} for simplicity.



